Coulomb Blockade in a Coupled Nanomechanical Electron Shuttle

We demonstrate single electron shuttling through two coupled nanomechanical pendula. The pendula are realized as nanopillars etched out of the semiconductor substrate. Coulomb blockade is found at room temperature, allowing metrological applications. By controlling the mechanical shuttling frequency we are able to validate the different regimes of electron shuttling.

==> 0457897.tex <==
%auto-ignore
